Deep Bayesian Active Learning for Preference Modeling in Large Language Models

Leveraging human preferences for steering the behavior of Large Language Models (LLMs) has demonstrated notable success in recent years. Nonetheless, data selection and labeling are still a bottleneck for these systems, particularly at large scale. Hence, selecting the most informative points for acquiring human feedback may considerably reduce the cost of preference labeling and unleash the further development of LLMs. Bayesian Active Learning provides a principled framework for addressing this challenge and has demonstrated remarkable success in diverse settings. However, previous attempts to employ it for Preference Modeling did not meet such expectations. In this work, we identify that naive epistemic uncertainty estimation leads to the acquisition of redundant samples. We address this by proposing the Bayesian Active Learner for Preference Modeling (BAL-PM), a novel stochastic acquisition policy that not only targets points of high epistemic uncertainty according to the preference model but also seeks to maximize the entropy of the acquired prompt distribution in the feature space spanned by the employed LLM. Notably, our experiments demonstrate that BAL-PM requires 33% to 68% fewer preference labels in two popular human preference datasets and exceeds previous stochastic Bayesian acquisition policies.

==> Tables/bald_batch.tex <==
\setlength{\intextsep}{0pt}%
\begin{table}[H]
% \renewcommand{\arraystretch}{2.5}
\begin{tabular}{l}
\toprule
\thead{BALD -- Acquired Batch} \\
\midrule
A bit of backstory: I've been in only 4 real long term relationships in my past.... \\
A bit of backstory: I've been in only 4 real long term relationships in my past.... \\
A bit of backstory: I've been in only 4 real long term relationships in my past.... \\
A few weeks ago my wife admitted to me that my best friend, (let's call him Marc... \\
A week ago I called off my relationship with my partner for a number of reasons,... \\
About a month ago my (23 F) boyfriend (26 M) of three and a half years and I got... \\
After 8 months my girlfriend decided to break up with me. Shes a very nice girl ... \\
For starters, its been awhile loseit, and I missed you! Things have been crazzzy... \\
For starters, its been awhile loseit, and I missed you! Things have been crazzzy... \\
For starters, its been awhile loseit, and I missed you! Things have been crazzzy... \\
For starters, its been awhile loseit, and I missed you! Things have been crazzzy... \\
Hello all I need some help regarding a friend of mine and a dream she had, well ... \\
Hello everyone, I am a student at a boarding school which means I am away from m... \\
Hi all. I am using a throwaway. I am 29f and my boyfriend is 32m. We have been d... \\
Hi all. I am using a throwaway. I am 29f and my boyfriend is 32m. We have been d... \\
Hi all. I am using a throwaway. I am 29f and my boyfriend is 32m. We have been d... \\
Hi first time user, and I am dyslexic so please forgive any spelling errors.   T... \\
I am 31 years old and currently live in New York. I have been a professional tre... \\
I was sitting on a bus and the seat beside me was empty..  A young nun walked do... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I work inside of a bread depot, and the drivers are effectively brokers, or our ... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
I've been married to my husband for 3 years, it's been wonderful, I couldn't ask... \\
It was my school's annual 5K, so the runners are students, faculty, and then ran... \\
% Ive worked with this girl once a week for almost a year. When we met we were bot... \\
% Ive worked with this girl once a week for almost a year. When we met we were bot... \\
% Ive worked with this girl once a week for almost a year. When we met we were bot... \\
% Ive worked with this girl once a week for almost a year. When we met we were bot... \\
% Ive worked with this girl once a week for almost a year. When we met we were bot... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
% My girlfriend and I have been going out for about a year and have decided to mov... \\
\bottomrule
\end{tabular}
\captionsetup{skip=5pt}
\caption{\textbf{First Acquired Batch by BALD (baseline)}.}
\label{tab:bald}
\end{table}

==> Tables/balpm_batch.tex <==
\setlength{\intextsep}{10pt}%
\begin{table}[t]
% \renewcommand{\arraystretch}{2.5}
\begin{tabular}{l}
\toprule
\thead{BAL-PM -- Acquired Batch} \\
\midrule
**Quick Background**: As the title states, we've been together for 7 years datin... \\
**The texts:**  Him: at least my mom thinks I'm cute  me: I think you're cute ;)... \\
**Warning: Avoid this film if you only broke up very recently! I advise this fil... \\
**i(26m) have been dating her(26f) on and off for 5 years.**  I have come to the... \\
--- So we broke up as in words she had severe depression and it wasn't fair to m... \\
A little while back, my sister asked me why some men were homophobic.  I answere... \\
A small background.  I live in in Puerto Rico, where I haven't had to good an ex... \\
About a month ago we started having problems with our cable. The picture would g... \\
Background info: Little background. I started medical school a few years back. I... \\
Backstory: I'm a 17 year old student in the U.K. currently in sixth-form. Back i... \\
Basically the above. He's 20. She's 15. Her parents are fucking lunatics and don... \\
Be sure to explain in detail with line breaks.  Hey my name is Matt and i honest... \\
Because I live in a very conservative Catholic neighborhood, I cannot come out a... \\
Been dating since february 2008. Sex was amazing, relationship was amazing unti ... \\
Hello all, Story:      I played around with some stocks a few years back buying ... \\
Hello reddit  My LDR girlfriend of six months told me yesterday that she wasn't ... \\
Hello!   Last group of friends I had was back in 10th Grade. Since then my depre... \\
Hello! I'm a 23 y/o F dating a 30 y/o male. This is by far the best relationship... \\
Hello, I'm kind of new to this sub reddit but I figured I'd get an opinion from ... \\
Hey Reddit. I spent at least 20 mins looking for the correct sub-reddit for men'... \\
Hey all. My classmates and I at the SUNY Purchase Film Conservatory are in the p... \\
Hey everyone so I'm about 3 months in of my 6 month regimen before I get gastric... \\
Hey fellow revenge-lovers, here's a quick one, that happened about an hour ago. ... \\
Hey guys this is strange to begin with, but I''ll introduce the situation:  I'm ... \\
I am a 24 y/o male and I have been dating a girl who is 22 years old for about 1... \\
I am an 18 year old college student and I have no attachments to my local area. ... \\
I am aware that this has been proposed before. I personally believe that it woul... \\
I am dating a complete dime like I get compliments all the time about her from s... \\
I can't focus. I can't become and remain motivated. When I've learned something ... \\
I know we are young but bear with me, I didn't know where else to go for this ty... \\
I live in California and am the co-owner of a car, with the names on the title b... \\
I made a previous post here but it sounded kind of stupid with the way I phrased... \\
I met my current girlfriend in highschool.  She's the only woman I've ever been ... \\
I should start with saying neither of us have had a chance to travel anywhere ex... \\
I want to start off by saying I love my SO and I'm looking for suggestions befor... \\
I was in a pretty serious car accident this week, and my car was easily totaled.... \\
I will try to make this as short as possible.  a long time ago i met this girl, ... \\
I work for Timezone, an arcade company opened to many places. A rude bitch walks... \\
I'll keep it short :3  I'm 18, he's 18. Dating for 3 years. When we walk togethe... \\
I'll keep this as succinct as possible.  I moved in Sept. 1. I used to live here... \\
I've been with my boyfriend for 4 years, it hasn't been the best relationship, b... \\
I've been with my gf for almost 7 years. Lived together for about 5 years. A few... \\
I've been working with this girl for 2 months. it started at work where i was he... \\
If you want to understand the scam, here's what's happening:  Okay, so I found a... \\
Im 27. Single. I am a productive member of society. I work full time i pay my ow... \\
It was New Year's Eve and my family was driving off to my grandparents' house. H... \\
It wasn't that long term relationships but we lived together for 6 months so we ... \\
Just got the new Kobo touch and they provided me with a \$10 gift card for their ... \\
My friend's little brother is really suffering in his dorm. He's lost 15-20 poun... \\
My girlfriend an I have been dating for three years. Its been the best time of m... \\
My girlfriend and I met through family friends a year and a half ago. We've been... \\
\bottomrule
\end{tabular}
\captionsetup{skip=0pt}
\caption{\textbf{First Acquired Batch by BAL-PM}.}
\label{tab:balpm}
\end{table}
